Galaxy Zoo: Morphological Classifications for 120,000 Galaxies in HST Legacy Imaging

We present the data release paper for the Galaxy Zoo: Hubble (GZH) project. This is the third phase in a large effort to measure reliable, detailed morphologies of galaxies by using crowdsourced visual classifications of colour composite images. Images in GZH were selected from various publicly-released Hubble Space Telescope Legacy programs conducted with the Advanced Camera for Surveys, with filters that probe the rest-frame optical emission from galaxies out to $z \sim 1$. The bulk of the sample is selected to have $m_{I814W} < 23.5$,but goes as faint as $m_{I814W} < 26.8$ for deep images combined over 5 epochs. The median redshift of the combined samples is $z = 0.9 \pm 0.6$, with a tail extending out to $z \sim 4$. The GZH morphological data include measurements of both bulge- and disk-dominated galaxies, details on spiral disk structure that relate to the Hubble type, bar identification, and numerous measurements of clump identification and geometry. This paper also describes a new method for calibrating morphologies for galaxies of different luminosities and at different redshifts by using artificially-redshifted galaxy images as a baseline. The GZH catalogue contains both raw and calibrated morphological vote fractions for 119,849 galaxies, providing the largest dataset to date suitable for large-scale studies of galaxy evolution out to $z \sim 1$.

==> ferengi.tex <==
\begin{table}
\caption{Summary of \ferengi{} artificial redshifting \label{tbl:ferengivalues}}
\begin{tabular}{lccccr}
\hline\hline
$z_{\rm sim}$ & $N_{z {\rm bins}}$ & $N_{\rm evolution}$ & $e_{\rm max}$ & $N_{\rm galaxies}$ & $N_{\rm images}$\\
\hline
0.3              & 8                  & 7                   & $-3.0$        & 72             & 4032 \\
0.5              & 6                  & 4                   & $-1.5$        & 72             & 1728 \\
0.8              & 3                  & 3                   & $-1.0$        & 72             &  648 \\
1.0              & 1                  & 3                   & $-1.0$        & 72             &  216 \\
\hline\hline
\end{tabular}
\end{table}


==> morphologies.tex <==
\begin{table*}
\center
\caption{Summary of morphological categories selected for \ferengi{} sample.\label{tbl:morphologies}}
\begin{tabular}{lllc}
\hline\hline
Morphology          & Label &  Selection                                                                                            & $N_{\rm objects}$ \\
                    &       &                                                                                                       & [$N_z \times N_\mu$] \\
\hline
Features            & Yes       & $f_{\rm features} > 0.8$, $f_{\rm odd} < 0.1$                                                         & 12 \\ 
                    & Int.      & $0.3 < f_{\rm smooth} < 0.6$, $f_{\rm odd} < 0.1$                                                     & 12 \\ 
                    & No        & $f_{\rm smooth} > 0.8$, $f_{\rm odd} < 0.1$                                                           & 12 \\ 
Merger              & No        & $f_{\rm features} > 0.8$, $f_{\rm odd < 0.1}$, $f_{\rm merger} < 0.1$                                 & 12 \\
                    & Int.      & $f_{\rm odd} > 0.5$, $0.1< f_{\rm merger} < 0.4$                                                      & 12 \\ 
                    & Yes       & $f_{\rm odd} > 0.5$, $f_{\rm merger} > 0.4$                                                           & 12 \\
Edge-on             & Yes       & $f_{\rm edgeon} > 0.8$, $f_{\rm features} > 0.5$                                                      & 12 \\
                    & Int.      & $0.4 < f_{\rm edgeon} < 0.8$ , $f_{\rm features} > 0.5$                                               & 12 \\
                    & No        & $f_{\rm edgeon} < 0.2$, $f_{\rm features} > 0.5$                                                      & 12 \\
Bar                 & No        & $f_{\rm bar} < 0.1$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$                                 & 24 \\
                    & Int.      & $0.2 < f_{\rm bar} < 0.4$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$                           & 24 \\
                    & Yes       & $f_{\rm bar} > 0.8$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$                                 & 24 \\
Visible spiral      & No        & $f_{\rm spiral} < 0.2$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$, $f_{\rm bar} < 0.1$         & 12 \\
                    & Int.      & $0.2 < f_{\rm spiral} < 0.8$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$, $f_{\rm bar} < 0.1$   & 12 \\
                    & Yes       & $f_{\rm spiral} > 0.8$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.2$, $f_{\rm bar} < 0.1$         & 12 \\
Oblique bulge size  & No        & $f_{\rm nobulge>0.6}$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.5$, $f_{\rm bar} < 0.2$          & 12 \\
                    & Int.      & $f_{\rm justnoticeable}>0.6$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.5$, $f_{\rm bar} < 0.2$   & 12 \\
                    & Yes       & $f_{\rm obvious|dominant}>0.5$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} < 0.5$, $f_{\rm bar} < 0.2$ & 12 \\
Edge-on bulge shape & Round     & $f_{\rm rounded}>0.5$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} > 0.5$                               & 12 \\
                    & Boxy      & $f_{\rm boxy}>0.4$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} > 0.2$                                  & 12 \\
                    & No bulge  & $f_{\rm nobulge}>0.5$, $f_{\rm features} > 0.5$, $f_{\rm edgeon} > 0.5$                               & 12 \\
\hline\hline
\end{tabular}
\end{table*}


==> redshifts.tex <==
\tabletypesize{\scriptsize}
\begin{deluxetable}{l|rr|rrr|rr|r|rr}
\tablecolumns{12}
\tablewidth{0pc}
\tablecaption{GZH redshifts by survey\label{tbl:redshifts}} 
\tabletypesize{\scriptsize}
\tablehead{
 &   
\multicolumn{2}{c}{\underline{ACS-GC}} &
\multicolumn{3}{c}{\underline{3DHST}} &
\multicolumn{2}{c}{\underline{MUSYC}} &
\multicolumn{1}{c}{\underline{UltraVISTA}}&
\multicolumn{2}{c}{\underline{Total}} 
\\
\colhead{Survey} & 
\colhead{spec-z} & 
\colhead{photo-z} & 
\colhead{spec-z} & 
\colhead{grism-z} & 
\colhead{photo-z} & 
\colhead{spec-z} & 
\colhead{photo-z} & 
\colhead{photo-z} & 
\colhead{with redshift} &
\colhead{in survey}
}
\small
\startdata
%Survey     Gs        Gp    3ds    3dg     3dp       Ms      Mp       UVp       total
AEGIS    & 3,656  & 2,941  & 12  &  515  &  249    & 0     & 0     &  0      & 7,373   & 8,507   \\
COSMOS   & 7,201  & 77,435 & 35  &  358  &  26     & 0     & 0     &  2,665  & 85,020  & 92,808  \\
GEMS     & 387    & 628    & 6   &  99   &  40     & 279   & 7,304 & 0       & 8,743   & 9,304   \\
GOODS-N  & 1,947  & 37     & 418 & 1,545 &  1,381  & 0     & 0     & 0       & 5,328   & 12,030  \\
GOODS-S  & 1,080  & 4      & 327 & 1,348 &  281    & 816   & 1,184 & 0       & 5,040   & 10,284  \\
SDSS     & 0      & 0      & 0   &  0    &  0      & 0     & 0     & 0       & 37,545  & 51,861  \\
\hline
Total    & 14,271 & 81,045 & 798 & 3,865 & 1,977   & 1,095 & 8,488 & 2,665   & 114,204 & 184,794 \\
\enddata
\end{deluxetable}

